Efficient representations for team and imperfect-recall equilibrium computation

Equilibrium finding in two-player zero-sum games with perfect recall is a well-studied topic that has led to many breakthroughs in computational game theory. This paper aims to generalize such techniques to (timeable) two-player zero-sum games with imperfect recall, or equivalently to two-team zero-sum games. In this setting, the problem of computing a mixed-strategy Nash equilibrium (or, equivalently, a team maxmin equilibrium with correlation) is known to be NP-hard. We connect the imperfect-recall setting with its perfect-recall counterpart through a novel construction we call the belief game. This is a perfect-recall game equivalent to a given (timeable) two-player zero-sum game with imperfect recall. The belief game may be exponentially larger than the original game but can be solved using any standard method. We then show that the strategy spaces of the two players in the belief game can be directly represented as a DAG, leading to a possibly exponential speedup. We call this the team belief DAG (TB-DAG). The TB-DAG simultaneously enjoys essentially optimal parameterized complexity bounds and the advantages of efficient regret minimization techniques. Along the way, we show $\Delta_2^P$-completeness and $\Sigma_2^P$-completeness of finding Nash equilibria in both mixed and behavioral strategies for the class of games we consider. Experimentally, we show that the TB-DAG, when paired with existing learning techniques, yields state-of-the-art performance on a wide variety of benchmark team games.

==> defs.tex <==
\newcommand{\commentsymbol}{\it\color{gray}$\triangleright$~}
\algrenewcommand\algorithmiccomment[1]{\hfill{\commentsymbol#1}}

\makeatletter
\newcommand{\LComment}[1]{\Statei {\commentsymbol{#1}}}
\newcommand{\Statei}{\Statex \hskip\ALG@thistlm}
\makeatother


\makeatletter
\autonum@generatePatchedReferenceCSL{Cref}
\autonum@generatePatchedReferenceCSL{cref}
\makeatother

\newcommand{\Crefdefpart}[2]{%
  \nameCref{#1}~\hyperref[#1]{\labelcref*{#1}.\ref*{#2}}%
}

\newcounter{Hequation}
\renewcommand{\theHequation}{\thesection.\arabic{Hequation}}
\makeatletter
\g@addto@macro\equation{\stepcounter{Hequation}}
\makeatother

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\ext}{\mathrm{ext}}
\let\E\relax
\DeclareMathOperator*{\E}{\mathbb{E}}

\newcommand{\splittwocols}[2]{%
\noindent\begin{minipage}{.5\linewidth}
        #1
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
        #2
    \end{minipage}
}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\textcolor{blue}{\emph{e.g}\onedot}}
\def\Eg{\textcolor{blue}{\emph{E.g}\onedot}}
\def\ie{\textcolor{blue}{\emph{i.e}\onedot}}
\def\Ie{\textcolor{blue}{\emph{I.e}\onedot}}
\def\cf{\textcolor{blue}{\emph{c.f}\onedot}}
\def\Cf{\textcolor{blue}{\emph{C.f}\onedot}}
\def\etc{\textcolor{blue}{\emph{etc}\onedot}}
\def\vs{\textcolor{blue}{\emph{vs}\onedot}}
\def\wrt{\textcolor{blue}{w.r.t\onedot}}
\def\dof{\textcolor{blue}{d.o.f\onedot}}
\def\etal{\textcolor{blue}{\emph{et }al}\onedot}
\makeatother

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{property}[theorem]{Property}
\crefname{property}{Property}{Properties}


\newcommand{\Reals}{\mathbb{R}}
\newcommand{\team}{\mathcal{T}}
\newcommand{\St}{\mathcal{S}}
\newcommand{\Ob}{\mathcal{O}}
\newcommand{\B}{\mathcal{B}}
\renewcommand{\C}{\mathcal{C}}
\newcommand{\avec}{\boldsymbol{a}}
\newcommand{\xvec}{\boldsymbol{x}}
\newcommand{\yvec}{\boldsymbol{y}}
\renewcommand{\co}{\op{co}}

\newcommand{\algoname}[1]{\textnormal{\textsc{#1}}}

\let\Root\varnothing
\let\R\Reals
\let\mc\mathcal
\let\op\operatorname
\let\ip\ev
\newcommand{\st}{\mathop{s.t.}}

\renewcommand{\H}{\ensuremath{\mathcal{H}}\xspace}
\newcommand{\N}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\I}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\Z}{\ensuremath{\mathcal{Z}}\xspace}
\renewcommand{\A}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\X}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\Y}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\J}{\ensuremath{\mathcal{J}}\xspace}
\renewcommand{\K}{\ensuremath{\mathcal{K}}\xspace}
\renewcommand{\S}{\ensuremath{\mathcal{S}}\xspace}

\newcommand{\vx}{{\vec x}}
\newcommand{\vy}{{\vec y}}
\newcommand{\vpi}{{\vec\pi}}
\let\vu\relax
\let\va\relax
\newcommand{\vu}{{\vec u}}
\newcommand{\va}{{\vec a}}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {\scriptsize #1};}}

\renewcommand\vec\boldsymbol
\renewcommand\emptyset\varnothing
\newcommand{\treepath}[2]{{\ensuremath{{#1} \to {#2}}}}
\newcommand{\splitb}[1]{\ensuremath{\algoname{SplitBelief}_{#1}}}
\newcommand{\LI}{\ensuremath{\operatorname{LI}}}
\newcommand{\cbox}[2]{\fcolorbox{white}[rgb]{#1}{\phantom{28m 13s}\llap{#2}}}
\newcommand{\unk}{\textcolor{black!30}{---}}
\makeatletter
\let\zz\Gscale@box
\long\def\Gscale@box#1{%
\xdef\thelastscalefactor{#1}%
\zz{#1}}

\makeatother
\DeclareRobustCommand{\thecolorscale}{\raisebox{-3.2mm}{\includegraphics[scale=.65]{figures/colorbar-crop.pdf}}}
\colorlet{teamcol}{gray}
\newcommand{\teamprint}[1]{\{\textcolor{teamcol}{#1}\}}
\newcommand{\nature}{{\ensuremath{0}}\xspace}
\newcommand{\donothing}{{\ensuremath{\diamond}}\xspace}

\makeatletter
\newcommand{\fsize}{\f@size}
\makeatother

\newcommand{\pmax}{{\ensuremath{\color{pmaxcolor}\blacktriangle}}\xspace}
\newcommand{\pmin}{{\ensuremath{\color{pmincolor}\blacktriangledown}}\xspace}
\newcommand{\tmax}{\text{\rotatebox[origin=c]{180}{\color{pmaxcolor}\ensuremath{\bm\triangledown}}}\xspace}
\newcommand{\tmin}{{\ensuremath{\color{pmincolor}\bm\triangledown}}\xspace}
\definecolor{pmaxcolor}{RGB}{31,119,180}
\definecolor{pmincolor}{RGB}{255,127,14}

\definecolor{p0color}{RGB}{0,0,0}
\definecolor{p1color}{RGB}{31,119,180}
\definecolor{p2color}{RGB}{255,127,14}
\newcommand{\sfbf}[1]{\textbf{\textsf{#1}}}
\newcommand{\util}[2]{\sfbf{{\color{p#1color}#2}}}

\newcommand{\nb}[3]{{\colorbox{#2}{\bfseries\sffamily\scriptsize\textcolor{white}{#1}}}{\textcolor{#2}{\sf\small\textit{~#3}}}}
\definecolor{mygreen}{rgb}{0.0, 0.5, 0.0}


\definecolor{briancolor}{rgb}{0.0, 0.82, 0.87}
\newcommand{\lu}[1]{\nb{Luca}{blue}{#1}}
\newcommand{\br}[1]{\nb{Brian}{briancolor}{#1}}
\newcommand{\fe}[1]{\nb{Federico}{mygreen}{#1}}
\newcommand{\nc}[1]{\nb{Nicola}{violet}{#1}}
\newcommand{\ga}[1]{\nb{Gabriele}{orange}{#1}}
\newcommand{\ju}[1]{\nb{Junkang}{purple}{#1}}

\let\eps\varepsilon

\newcommand{\namealg}[1]{\renewcommand{\thealgorithm}{\tt #1}}
\captionsetup[algorithm]{labelsep=colon}

\newcommand\changed[1]{{#1}}

